Mice with finitely many Woodin cardinals from optimal determinacy hypotheses

We prove the following result which is due to the third author. Let $n \geq 1$. If $\boldsymbol\Pi^1_n$ determinacy and $\Pi^1_{n+1}$ determinacy both hold true and there is no $\boldsymbol\Sigma^1_{n+2}$-definable $\omega_1$-sequence of pairwise distinct reals, then $M_n^\#$ exists and is $\omega_1$-iterable. The proof yields that $\boldsymbol\Pi^1_{n+1}$ determinacy implies that $M_n^\#(x)$ exists and is $\omega_1$-iterable for all reals $x$. A consequence is the Determinacy Transfer Theorem for arbitrary $n \geq 1$, namely the statement that $\boldsymbol\Pi^1_{n+1}$ determinacy implies $\Game^{(n)}(<\omega^2 - \boldsymbol\Pi^1_1)$ determinacy.

==> Conclusion.tex <==


For sets of reals in $L(\R)$ we finally proved the following theorem
in this part of the thesis.

\begin{thm}
  \label{thm:LR1}
  Let $\alpha < \beta$ be ordinals such that $[\alpha, \beta]$ is a
  weak $\Sigma_1$-gap and let
  \[ A \in \Gamma = \SIGMA_n(J_\beta(\R)) \cap \Pot(\R), \]
  where $n < \omega$ is the least natural number such that
  $\rho_n(J_\beta(\R)) = \R$.  Moreover assume that every
  $\PI^1_5\Gamma$-definable set of reals is determined.  Then there
  exists an $\omega_1$-iterable hybrid $\Sigma$-premouse $\N$ which
  captures $A$.
\end{thm}

\begin{proof}
  If we let $\N = M_1^{\Sigma, \#}$ this follows from Corollary
  \ref{cor:mainResultHybrid} together with Corollary
  \ref{cor:projcapturing} and Theorem \ref{thm:obtainFittingPair}.
\end{proof}

In fact we showed the following more general theorem, which also
follows from Corollary \ref{cor:mainResultHybrid} together with
Corollary \ref{cor:projcapturing} and Theorem
\ref{thm:obtainFittingPair}.

\begin{thm}
  \label{thm:LR2}
  Let $\alpha < \beta$ be ordinals such that $[\alpha, \beta]$ is a
  weak $\Sigma_1$-gap, let $k \geq 0$, and let
  \[ A \in \Gamma = \SIGMA_n(J_\beta(\R)) \cap \Pot(\R), \]where
  $n < \omega$ is the least natural number such that
  $\rho_n(J_\beta(\R)) = \R$. Moreover assume that every
  $\PI^1_{2k+5}\Gamma$-definable set of reals is determined.  Then
  there exists an $\omega_1$-iterable hybrid $\Sigma$-premouse $\N$
  which captures every set of reals in the pointclass $\Sigma^1_k(A)$
  or $\Pi^1_k(A)$.
\end{thm}

Here we again denote by $\Sigma^1_n(A)$ and $\Pi^1_n(A)$ for
$n < \omega$ and a set of reals $A$ the set of all reals which are
definable over the model $(V_{\omega+1}, \in, A)$ by a $\Sigma_n$- or
a $\Pi_n$-formula respectively from the parameter $V_{\omega+1}$.

Converse directions of the results presented in this part of the
thesis, for example obtaining determinacy for sets of reals in levels
of the $L(\R)$-hierarchy from the existence and $\omega_1$-iterability
of the $\Sigma$-premouse $M_k^{\Sigma,\#}$ for $k<\omega$ and an
iteration strategy $\Sigma$ which condenses well for some appropriate
countable premouse $\N$, are due to Itay Neeman and follow from
\cite{Ne02} (see Definition $2.10$ and Theorem $2.14$ in \cite{Ne02}).

\section{Open Problems}
\label{sec:openproblemsHybrid}

We close with mentioning some related open problems. The result we
proved in this part of the thesis concerning sets in the
$L(\R)$-hierarchy is most likely not optimal, but at some levels in
the $L(\R)$-hierarchy it it is not even clear which mice to consider
when aiming for an optimal result. 

A promising candidate would be a mouse whose \emph{mouse
  set}\index{mouse set} is definable in a countable ordinal over a
level of the $L(\R)$-hierarchy, where a mouse set as defined by
Mitchell Rudominer is the set of reals of a mouse. This would mimic
the situation in the projective hierarchy since there we have the
following theorem.

\begin{thm}[Martin, Steel, Woodin in \cite{St95}]
  Let $n \geq 1$ and assume that $M_n^\#$ exists and is
  $\omega_1$-iterable. Then $\R \cap M_n^\#$ is exactly the set of
  reals which are $\Delta^1_{n+2}$-definable in a countable ordinal.
\end{thm}

Mitch Rudominer investigated mouse sets in the $L(\R)$-hierarchy in
\cite{Ru97}. But for some levels of the $L(\R)$-hierarchy, for example
for the set of reals which are $\Delta_2$-definable in a countable
ordinal over the first level after the projective sets $J_2(\R)$, the
question what the right mouse to consider is remains open.

All definitions and results which we describe concerning this question
are due to Rudominer and can be found in \cite{Ru97}.  It is
conjectured that the right candidate at this level is a so called
ladder mouse, which is defined as follows.

\begin{definition}
  A mouse $\mathcal{P}$ is called a \emph{ladder mouse} \index{ladder
    mouse} iff there exists a sequence $(\delta_n \st n < \omega)$ of
  cardinals in $\mathcal{P}$ such that
  $\mathcal{P} \cap \Ord = \sup_{n<\omega} \delta_n$ and we have for
  all $n < \omega$ that
  \begin{enumerate}[$(1)$]
  \item
    $M_n^\#(\mathcal{P} | \delta_n) \vDash \text{``}\delta_n \text{ is
      a Woodin cardinal''}$, and
  \item  $M_n^\#(\mathcal{P} | \delta_n) \unlhd \mathcal{P}$.
  \end{enumerate}
\end{definition}

So the following is conjectured.

\begin{conj}[Steel, Woodin, 2015]
  Let $\mathcal{P}$ be the minimal ladder mouse. Then for all reals
  $x$, we have that
  \[ x \in \mathcal{P} \cap \R \text{ iff } x \text{ is }
  \Delta_2(J_2(\R)) \text{-definable in a countable ordinal.} \]
\end{conj}

What is known so far is, that the minimal ladder mouse as defined
above is a lower bound for the set of reals which are
$\Delta_2(J_2(\R))$-definable in a countable ordinal.

\begin{thm}[Rudominer in \cite{Ru97}]
  Let $\mathcal{P}$ be the minimal ladder mouse and let
  $x \in \mathcal{P} \cap \R$. Then $x$ is
  $\Delta_2(J_2(\R))$-definable in a countable ordinal.
\end{thm}

The known upper bound for the set of reals which are
$\Delta_2(J_2(\R))$-definable in a countable ordinal is an admissible
ladder mouse, which is defined as follows. 

\begin{definition}
  A mouse $\mathcal{P}_a$ is called an \emph{admissible ladder mouse}
  \index{admissible ladder mouse} iff there exists a sequence
  $(\delta_n \st n < \omega)$ of cardinals in $\mathcal{P}_a$ such
  that $\mathcal{P}_a \cap \Ord$ is the least admissible ordinal above
  $\sup_{n<\omega} \delta_n$ and we have for all $n < \omega$ that
  \begin{enumerate}[$(1)$]
  \item
    $M_n^\#(\mathcal{P}_a | \delta_n) \vDash \text{``}\delta_n \text{ is
      a Woodin cardinal''}$, and
  \item  $M_n^\#(\mathcal{P}_a | \delta_n) \unlhd \mathcal{P}_a$.
  \end{enumerate}
\end{definition}

\begin{thm}[Rudominer in \cite{Ru97}]
  Let $\mathcal{P}_a$ be the minimal admissible ladder mouse and let
  $x$ be a real which is $\Delta_2(J_2(\R))$-definable in a countable
  ordinal. Then $x \in \mathcal{P}_a$. 
\end{thm}

So there are still lots of interesting questions concerning
generalizations of results in the projective hierarchy to levels of
the $L(\R)$-hierarchy which remain open and further research has to be
done to analyse the full picture of the sets of reals in the
$L(\R)$-hierarchy and their connection to mice.



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "Main"
%%% End:


==> ConseqDet.tex <==

In what follows we will need the following consequence of determinacy
which is an analogue of Lemma \ref{lem:bfDetSeq}. 

\begin{thm}
  \label{thm:defseqctble}
  Let $k < \omega$ and let $\N$ be a countable premouse and $\Sigma$
  an $\omega_1$-iteration strategy for $\N$ which condenses
  well. Moreover let $\Gamma$ be a pointclass which is
  $(\N, \Sigma)$-apt. Assume that every
  $\PI^1_{2k+3} \Gamma$-definable set of reals is determined. Then
  there exists no uncountable $\SIGMA^1_{2k+4} \Gamma$-definable
  sequence of pairwise distinct reals.
\end{thm}

\begin{remark}
  The statement ``there exists no uncountable
  $\SIGMA^1_{2k+4} \Gamma$-definable sequence of pairwise distinct
  reals'' is defined analogous to Part 1 (see remark after the
  statement of Theorem \ref{thm:newWoodin1}).
\end{remark}

\begin{proof}[Proof of Theorem \ref{thm:defseqctble}]
  The proof of this theorem is analogous to the descriptive set
  theoretic argument for the odd levels of the projective hierarchy in
  the proof of Lemma \ref{lem:bfDetSeq}. We will present it here to
  convince the reader, that it also works in this setting with some
  minor adjustments. Note that the inner model theoretic argument we
  gave for the even levels of the projective hierarchy in the proof of
  Lemma \ref{lem:bfDetSeq} does not work here, because at the moment
  we are not able to construct hybrid premice which are suitable
  enough to apply this argument from the amount of determinacy we are
  assuming.

  Assume toward a contradiction that there exists a
  $\SIGMA^1_{2k+4} \Gamma$-definable $\omega_1$-sequence of pairwise
  distinct reals. That means in particular that there exists a
  well-order $\leq^*$ of ordertype $\omega_1$ for reals such that if
  we let $X_{\leq^*} = field(\leq^*)$, that means if we have for all
  $y \in \BS$,
  \[y \in X_{\leq^*} \; \Leftrightarrow \; \exists x \; (x \leq^* y
  \vee y \leq^* x), \]
  then there exists a $\SIGMA^1_{2k+4} \Gamma$-definable relation $R$
  such that we have for all $x,y \in \BS$,
  \[ R(x,y) \; \Leftrightarrow \; x,y \in X_{\leq^*} \; \wedge \; x
  \leq^* y. \]
  Let $A$ be a $\PI^1_{2k+3} \Gamma$-definable relation such that we
  have for all $x, y \in \BS$,
  \[ R(x,y) \; \Leftrightarrow \; \exists z \, A(z,x,y). \]

  Moreover consider the relation $A_2$ such that for all $u \in (\BS)^2$
  and for all $y \in \BS$, 
  \[ A_2(y,u) \; \Leftrightarrow \; A( (u)_0, (u)_1, y). \]

  Recall that we fixed $\Gamma$ such that the pointclass
  $\PI^1_{2k+3} \Gamma$ has the uniformization property. Therefore
  there exists a $\PI^1_{2k+3} \Gamma$-definable function $F$ which
  uniformizes the set $A_2$, that means we have
  \[ (y, F(y)) \in A_2 \]
  for all $y \in \dom(F)$.  We have that $X_{\leq^*} \subseteq
  \dom(F)$. So the relation $A^*$ defined by
  \[ A^*(z,x,y,u) \; \Leftrightarrow \; A(z,x,y) \wedge z = (u)_0
  \wedge x = (u)_1 \wedge u = F(y) \]
  is $\PI^1_{2k+3} \Gamma$-definable. Let $A^*$ denote the
  corresponding set of all tuples $(z,x,y,u)$ such that $A^*(z,x,y,u)$
  holds.

  As before we now consider the following game $G^p(A^*)$ which is due
  to M. Davis (see \cite{Da64} or Theorem $12.11$ in \cite{Sch14}). We
  again identify the elements of the set $A^*$ with elements of the
  Cantor space $^\omega 2$. 

  \begin{figure}[h]
    \centering
    \begin{tabular}{c|cccccc}
      $\mathrm{I}$ & $s_0$ & & $s_1$ & & $\dots$ \\ \hline
      $\mathrm{II}$ & & $n_0$ & & $n_1$ & & $\dots$ 
    \end{tabular}
  \end{figure}

  Player $\mathrm{I}$ plays finite $0-1$-sequences
  $s_i \in {}^{<\omega}2$ (allowing $s_i = \emptyset$), player
  $\mathrm{II}$ responds with $n_i \in \{0,1\}$ and the game lasts
  $\omega$ steps. We say player $\mathrm{I}$ wins the game $G^p(A^*)$
  iff
  \[ s_0^{} {}^\frown n_0 {}^\frown s_1 {}^\frown n_1 {}^\frown \dots
  \in A^*. \]
  Otherwise player $\mathrm{II}$ wins. As a consequence of our
  determinacy hypothesis we have that the game $G^p(A^*)$ is
  determined, because we may code $G^p(A^*)$ into a Gale-Stewart game
  $G(A^\prime)$ for some set of reals $A^\prime$ which is
  $\PI^1_{2k+3}\Gamma$-definable.

  Then we can argue again as in the proof Theorem $12.11$ in
  \cite{Sch14} to obtain that the set $A^*$ has a perfect subset,
  because $A^*$ is uncountable. As in the proof of Lemma
  \ref{lem:bfDetSeq} this yields that we have the following claim.

  \begin{claim}
    The set
    \[ B = \{ y \st \exists z \exists x \exists u \; A^*(z,x,y,u)
    \} \] has a perfect subset.
  \end{claim}

  Therefore there exists a continuous function $f: \R \rightarrow B$
  and we can consider the following order $\leq$ on the reals. We say
  for two reals $x$ and $y$ that
  \[ x \leq y \Leftrightarrow f(x) \leq^* f(y). \]
  Then we again have the following claim. 

  \begin{claim}\label{cl:h-wo-reals}
    The order $\leq$ is a $\SIGMA^1_{2k+4} \Gamma$-definable
    well-order of the reals.
  \end{claim}

  We can now use this claim to prove the following claim exactly as in
  the proof of Lemma \ref{lem:bfDetSeq} with Bernstein's argument, so
  we omit the proof here.

  \begin{claim}
    There are two disjoint $\SIGMA^1_{2k+4} \Gamma$-definable sets $D$ and
    $D^\prime$ of size $\aleph_1$ without perfect subsets. 
  \end{claim}

  Let $E$ be a $\PI^1_{2k+3} \Gamma$-definable set such that
  \[ x \in D \; \Leftrightarrow \; \exists y \; (x,y) \in E. \]
  Since we assumed that $\PI^1_{2k+3} \Gamma$-uniformization holds,
  there exists a $\PI^1_{2k+3}\Gamma$-definable partial function
  $C: \R \rightarrow \R$ uniformizing $E$, that means we have that
  \[ \exists y \, (x,y) \in E \Leftrightarrow (x, C(x)) \in E. \]

  The set $C^\prime$ which is defined as
  \[ C^\prime = \{ (x, C(x)) \st x \in D \} = C \cap E \]
  is $\PI^1_{2k+3} \Gamma$-definable and consider the Davis game
  $G^p(C^\prime)$, which is again determined by assumption.

  As above this yields that $C^\prime$ has a perfect subset
  $P \subset C^\prime$, because $D$ and thus $C^\prime$ is
  uncountable.  Since $P$ is a perfect set and $D$ does not contain a
  perfect subset, there are reals $x,y$ and $y^\prime$ such that
  $y \neq y^\prime$ and $(x,y) \in P$ and $(x, y^\prime) \in P$. But
  we have $y = C(x) = y^\prime$. This is a contradiction.
\end{proof}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "Main"
%%% End:

